Marginal Contribution Feature Importance -- an Axiomatic Approach for The Natural Case

When training a predictive model over medical data, the goal is sometimes to gain insights about a certain disease. In such cases, it is common to use feature importance as a tool to highlight significant factors contributing to that disease. As there are many existing methods for computing feature importance scores, understanding their relative merits is not trivial. Further, the diversity of scenarios in which they are used lead to different expectations from the feature importance scores. While it is common to make the distinction between local scores that focus on individual predictions and global scores that look at the contribution of a feature to the model, another important division distinguishes model scenarios, in which the goal is to understand predictions of a given model from natural scenarios, in which the goal is to understand a phenomenon such as a disease. We develop a set of axioms that represent the properties expected from a feature importance function in the natural scenario and prove that there exists only one function that satisfies all of them, the Marginal Contribution Feature Importance (MCI). We analyze this function for its theoretical and empirical properties and compare it to other feature importance scores. While our focus is the natural scenario, we suggest that our axiomatic approach could be carried out in other scenarios too.

==> abstract.tex <==

The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.


==> definitions.tex <==
\section{Definitions}\label{Sec:Definitions}
\subsection{Global predictive power}
\scomment{I'm confused by the distinction between valuation function and global predictive power. Since the global predictive power is well-defined, are there multiple valuation functions for a given global predictive power. Or do we think of valuation function as possible candidates that approximate the global prediction?}
In this work, we would like to define the feature importance of $x_i \in X$ w.r.t to a target variable $Y$ as the amount of \emph{global predictive power} it contribute. This term is defined by~\cite{covert2020understanding} as follows: given a loss function $\ell$, the global predictive power of a set of features $S \subseteq F$ is a function $u: \mathcal{P}(F) \longrightarrow \R^+$, where $\mathcal{P}(F)$ is the power set of $F$. This function measures the expected loss reduction between the optimal predictor $f$ when it using $S$, and the optimal constant predictor $\hat{y}$, i.e: 
\[
u(S) = \min\limits_{\hat{y}} \mathop{\mathbb{E}}[\ell(\hat{y}, Y)] - \min_{g} \mathop{\mathbb{E}}[\ell(g(x), Y)] % we may add here a comment same 
\]
Where the expectation is taken over $p(x,y)$.\\
The \emph{predictive power} of a set of features is defined in context of a specific predictor $f$, $u_f: \mathcal{P}(F) \longrightarrow \R^+$:  
\[
u_f(S) = \min_{\hat{y}} E(l(\hat{y}, Y)) - E(l(f(x), Y))
\]

Alternative natural choices to define global predictive power might be mutual information or the expected accuracy of the optimal Bayesian predictor.

\subsection{Valuation function}

\begin{definition}
A  valuation function is any function $\nu: \mathcal{P}(F) \longrightarrow \R^+$ that satisfy the following properties:

\begin{enumerate}
    \item  \textbf{Has no bias}: $\nu\{\phi\} = 0$
    \item \textbf{Monotonic increasing with the set of features}: if $S \subseteq T \subseteq F$ then $\nu(S) \leq \nu(T)$
\end{enumerate}
\end{definition}

We assume that the above are desirable properties of any function that measures global predictive power, as adding features can only improve the optimal predictor, and it's reasonable to assume for normalization purpose that the empty set of features has no predictive power. From now on, we denote any valuation function that evaluates the global predictive power as $\nu$, and any valuation function that evaluates the predictive power of some model f as $\nu_f$.


==> impact.tex <==
\section{Broader Impact}\label{Sec:Impact}
In this work, we addressed an important scenario of feature importance in which the goal is to highlight significant factors that related to a certain phenomena in the real world such as a disease. The ability to assign accurate importance scores in this scenario can make impact in several important disciplines.

In biology for example, consider scientists trying to learn about a mechanism of a disease. Scientists can run experiments in the lab to test the influence of changes in different locations in the DNA on the disease, but such experiments are expensive and time-consuming. An accurate feature importance score could help them to better utilize their resources. 

In social science for example, consider researchers trying to understand social inequalities. Having in their disposal an accurate tool that highlights the most important factors impacting salaries for example, can help them identify important biases, such as biases related to gender or race. 

Further, we hope that our work will inspire other researchers to study the difference between the natural scenarios and the model scenarios and using the axiomatic approach.

==> results.tex <==
\section{Results}\label{Sec:Results}
